Walking Down the Road to Independent Mobility: An Adaptive Route Training System for the Cognitively Impaired

In this paper we describe the design and development of a route training system for individuals with cognitive impairments (CIs) living in residential care facilities. Learning to move autonomously in public spaces is a fundamental skill for people with CI, who face several challenges to independently and safely move around. Yet, exploring opportunities for route training support, especially in residential settings, has received very little attention. To explore these opportunities, we followed a design and development process based on inclusive design practices that considered the organisational context and aimed at involving people with CI in the software design. To ensure our solution addressed the identified needs and abilities of this heterogeneous population, we further framed the route training definition as a design process that is enacted by the system, making the trainer and user co-creators of a personalised training. In this paper we report on the needs and challenges for mobility training in residential settings, introduce the design and formative evaluation of the route training system, to conclude with reflections and considerations on our methodological approach.

==> sections/design.tex <==
\begin{figure*}[ht!]
  \centering
  \includegraphics[width=\linewidth]{figures/paganini-architecture.pdf}
  \caption{General training process illustrating the interaction points of the main actors with the system components}
  \Description{General training process illustrating the interaction points of the main actors with the system components.}
  \label{fig:architecture}
\end{figure*}

\section{System Design and Rationale}

The initial phase led to the design and development of a system to address the route training needs of the users in the organisational context. The system, namely PAGAnInI, aims at enabling individuals with CI to follow a personalised \textit{route training program} that can adapt to their goals, abilities and learning progress, while reducing negative feeling and risks associated to independently walking in public spaces. The training is overseen by a mobility trainer (e.g., a caregiver) who can steer, monitor or intervene in the training with the support of the system. Figure \ref{fig:architecture} illustrates how the users interact with the two main apps of the PAGAnInI system to carry out the route training. In the following, we elaborate on the system design and describe how it addresses the user needs and requirements.

% individuals with CI 
% driven by a expert fa

% Design concept
% an overview, explained in terms of main components
% and how these components address the main needs

% Process
%we should introduce the scenario (storyboard?) showing the entire training process, and how users interact with the different apps for this purpose.
% We paint an overview
% Check the requirements, and make sure they are informally address, as we will anyway go in detail in the subsections
% \begin{enumerate}
%     \item \ding{182} Exploratory route walk
%     \item Initial path definition
%     \item Path negotiation
%     \item Adaptive route training
%     \item Monitoring and assessment
    
% \end{enumerate}

% Supported by two applications
% An architecture 




% The design space:
% - how do we encode the training
% - how to facilitate the negotiation
% - how to deliver the wayfinding instructions

% --->> Introduce the conceptual model first? my concepts, etc

\subsection{Route training concepts}
% {\color{red}introduce concepts and conceptual model?

% What is route training. Why?

% Landmark-based navigation

% Landmark

% Reassurance

% Decision  point
% }

%Before delving into the main components of the system, we introduce the notion of route training and related concepts. 
\textit{Route training} is an important aspect of mobility training that focuses on training people in finding their way from a starting point to a destination (e.g., from home to work). People with CIs are challenged in their ability to abstract, generalise and transfer knowledge, so wayfinding requires rehearsing and learning each specific route with an individual instead of teaching general navigation strategies [xx]. As we have seen from our initial studies, 
%since this involves training each specific individual along specific routes, 
it is the training task that demands the most effort and commitment from professionals and organisations. In the context of the training, we will denote simply as \textit{user}, to individual with CIs that acts as trainee, and \textit{trainer} to the care professional that acts as mobility trainer.
Next, we introduce the main concepts of our training approach:




\begin{itemize}[leftmargin=10pt,topsep=5pt]

\item \textit{Way}. A way is the (street-)connection a user wants to be able to walk independently, e.g., to get home from work. 
%A way is defined by a starting point, an end point, a name, and a description. 
Ways are not bidirectional, as the impressions, scenery and instructions change with the direction of walk. 
%Ways can contain several routes.

\item \textit{Path}. One exact (street-)path to walk along in a specific way. A way can contain several possible paths that differ in distance, time, complexity, traffic situation, detours, etc.

\item \textit{Route}.
A path augmented with landmarks and reassurances that serves as the basis for route training.

\item \textit{POI}. Points of interest are places that stand out to the user during a route walk. These are marked during initial planning stage, as places that could be adopted as either landmarks or reassurances in the training. They consist of a coordinate, a timestamp, a type (e.g., landmark, reassurance) and at least one photo. 

\item \textit{Landmark}. POI that was negotiated with users and confirmed as a landmark. Landmarks are objects that are not subject to rapid change and may have a personal reference for the user (houses, trees...), where a decision must be made ("At the house where Peter lives, turn right onto the small footpath"). 

\item \textit{Reassurance}. POI that was negotiated as a reassurance. Reassurances are prominent points along a route (e.g., church tower, skyline, house, tree) where no decision must be made, but which encourage the user to be on the correct path and helps to remember the next landmark.

\end{itemize}


The above concepts are the basis for \textit{landmark-based} wayfinding. We adopted a landmark-based approach to support wayfinding, which is the preferred, less cognitively demanding and most effective approach for individuals with CIs according to previous studies [xx]. In this approach, the  idea is to rely on \textit{landmarks} along a route as primary means of providing direction and supporting decisions, rather than turn-by-turn directions. 

%Next we detail the training process depicted in Figure~\ref{fig:architecture}, along with the rationale of design decisions. 


% We might want to add a subsection here, like Process
% and highlight the main design principles behind the design of the system


\subsection{Route training system}

In this subsection we detail the training process depicted in Figure~\ref{fig:architecture}. We highlight the design space, the rationale behind design choices and ingredients of the system that resulted from our iterative process. This should note however that this but do not reflect the current status of the implementation. 


\fakeSection{Exploratory route walk}
In the context of the training, the first point of interaction with the system is the \textit{exploratory route walk}. This is a preliminary walking session with the trainer along the intended route, with the purpose of i) assessing the abilities of the user and the feasibility of walking independently along the route by leveraging his expertise and contextual knowledge (R2), and ii) collecting and eliciting relevant data for the definition of the route training.  This activity is supported by a component of the same name, in the PAGAnInI mobile app.

The walking session starts at the beginning of the route (e.g., Home) and ends at its destination (e.g., Work). The specific path to follow between the two points of the route is decided by the trainer based on the specific abilities, background and goals of the user (e.g., path featuring memorable characteristics, simpler or safer to navigate, faster). 
%usage and intended interaction
It is important to note that in the process of defining the route training, the trainer may explore different routes. 

During the walk, the system collects information necessary for the training. This includes i) \textit{GPS points} recorded along the way so as to reconstruct the path actually walked, ii) candidate \textit{landmarks} with pictures and additional notes, necessary to support landmark-based navigation (R5), and iii) \textit{video recording} of the walk to facilitate the analysis for the route definition and negotiation. GPS data and video are recorded automatically, but the landmark information should be elicited by the trainer based on their experience and best practices [\textbf{xx}]. 
%
As sensitive data is recorded during this process (video recording and pictures), all the information is stored on the local mobile phone of the user and transferred to the Trainer app through a peer to peer connection (R8). This information is curated by the trainer in the next step of the process (route definition), and synced to the cloud only then. Some information such as video recording is never synced to the server. 

% landmark based training (R5)
% data collection - what data and why
% Collect data for the definition of the personalised training and route definition

% - gps points, every 4 meters? - route actually walked (not generated by a system)
% - candidate landmarks, with pictures and additional material 
% - video recording of the walk for analysis

In terms of interaction design, this component of the system was designed to require minimal intervention (R9), with options limited to start and stop the recording, and capture landmarks along the way. It is designed to be used by either the trainer or the user, depending on the dynamics of their interactions.

%accessibility, design decisions here? (R9)
%- 


% sensitive data (R8)
% volume of data
% Synchronised directly to the 




% It starts with some walking sessions with the social worker to define a personalised path with landmarks, photos and additional material to ensure best learning outcomes


% Space to study the feasibility, and elaborate a plan of action
% Collect data for the definition of the personalised training and route definition


\fakeSection{Route definition and negotiation}
The next step in the process is the \textit{route definition}. In this phase the trainer analyses all the information collected in the exploratory route walk to curate a "prototype" route definition that can be later negotiated with the users. Unlike previous approaches that rely off-the-shelf navigation instructions or automatically generated landmarks \cite{kramer2015developing,ramos2013geo}, we rely on the trainer, their experience and feedback loops to define and personalise the route (R2,R3). This activity is supported by a component of the same name in the PAGAnInI Trainer app, which runs on tablet computers.

To support the analysis and reflection on the collected data, this component allows the Trainer to playback the entire exploratory route walk session. This is done by synchronising video playback, the walking progress on a map representation of the route, with markers on playback progress and the map signaling geotagged POI and pictures. With this visualisation, the user can not only replay the session, but also jump to any landmark or point along the way to watch / listen to the discussion around it. 
%
The Trainer can then curate the route definition. This implies adding, editing and removing POIs and pictures, curating instructions and adding notes for the discussion with the user. The actual path can also be edited, e.g., to fix potential GPS issues. 

% Curate the entire route definition
% curate (add / edit / remove) the landmarks and pictures, 
% define decision points and reasurances (R5)
% curate instructions
% and add notes for the route negotiation with the user.


Next, the prototype route definition is jointly discussed with the user in what we call the "negotiation", to derive a first working route definition that fits the individual. The \textit{negotiation} aims at involving the user in the definition of the route, extending the idea of inclusive design practices from software alone to the preparation of the training. Thus, there are two main goals to the negotiation: i) making sure we select appropriate route elements (e.g., landmarks) so as to maximise learning (e.g., is this a potentially effective landmark?), and ii) making sure the user would be able to follow the instructions, so as to maximise comprehension and understanding (e.g., are these instructions understandable?).

The system facilitates the route negotiation through a simplified version of the route definition interface, that uses a slideshow metaphor to go over POIs one by one, emphasising pictures and instructions. The Trainer should then elicit the required feedback on each POI, pictures and instructions to apply or annotate the feedback (e.g., confirm POI, tag picture as to-be changed). Following co-design practices that resulted effective in our own design process, we included an option to "preview" the route definition in a mock representation of the training app. By clicking on preview route, the Trainer can show users how the POI would be displayed during the training, thus eliciting feedback on concrete artefacts.





% synchronising the video
% the movement along a map representation of the path
% and markers displaying geotagged pictures and landmakrs.


% simplied version
% emphasise pictures
% and instructions cv
% mock presentation




% Negotiation

% Adaptation R3
% Setting up the training goals


% Negotiation

% Adaptation R3
% R7 abilities to learn


% ensure best learning outcomes



\fakeSection{Route training} 
The \textit{route training} is the actual learning activity, where the trainer and the user practice the negotiated route definition, working towards the increasing degree of independence and self-reliance of the user. To effectively accomplish this, the training should adapt to the interaction abilities, navigation skills and goals, and progress during the training.  
%
Our \textit{adaptive route training} approach thus considers three dimensions for adapting the training: i) degree of support, ii) type of instructions, and iii) interaction modality. 

% an overview of how it works the training here?

%To illustrate how these elements play together, 
Let us start by describing all these dimensions play together in the training. With the trainee app, the user follows the route definition from start to destination with a given \textit{degree of support} (e.g., assisted by an in-person human trainer). Wayfinding instructions are relied by leveraging specific \textit{strategies} (e.g., traditional landmark-based instructions) and displayed to the user in specific \textit{modalities} (e.g., text and audio). In the case of unexpected situations (e.g., user lost or confused) the system can prompt recovery options to assist the user. While practicing the route, the system collects relevant data to compute progress metrics and enable remote monitoring. In this subsection we describe how these dimensions modify the training, and in the next how the adaptation takes place.


The support provided by the trainer goes from in-person training support, and remote training support to system-based support. The starting point is \textit{in-person} support, where trainer assists the user in the landmark-based navigation of the route, using their mobility training expertise to increase the independence of the user to a point where it is safe for the user to practice the route on their own. Next, the trainer can provide a similar assistance via a \textit{remote} audio link supported via a monitoring interface. In the last degree of support, the training \textit{app takes over} the on-the-road training, with the trainer taking a passive role in monitoring the progress.

The second dimension to the adaptation is the type strategy used to relay instructions to the user. We rely on strategies that incrementally aim at removing the assistance provided by the app. \textit{Actionable mode} relay explicit guidance within the landmark-based navigation, notifying users of decision points and reassurances. The \textit{quiz mode}, inspired by the gamification approach in \cite{brown2013engaging}, prompts users about the way to go when reaching decision points. The quiz acts as a checkpoint that encourage attention and provide valuable signals to analyse the progress of the user. The \textit{reward mode} turns off instructions at decision points to provide retrospective feedback, rewarding users for making the correct decisions or alerting them of a mistakes made past the decision points. Finally, \textit{mute mode} turns off the assistance on a POI. It is important to note that these strategies can be applied to specific sub-paths along the way, and not only as a general strategy for the general route navigation (contrary to \cite{brown2013engaging}). In our prototyping experience, this emerged as an  aspect to address, since users have might have different level of familiarity or be more challenged by certain parts of the route.

The third dimension of the adaptation is the instruction modality. Given the different interaction and comprehension abilities, the interface rely on multiple representations including text, symbols (e.g., arrows, signals), audio, tactile and augmented reality (AR), which can be made available to the user under certain constraints for safety of use. 
%
Multimodal alerts are brought when in the vicinity of a POI to prevent users from staring at their phones waiting for visual feedback, and these cannot be changed or deactivated.\footnote{Deactivating alerts is done by modifying the relay strategy, e.g. mute mode.} AR  can only act as a supplementary modality. When in doubt, the user will activate the AR modality by lifting the phone and pointing the phone camera on the road, and as a result the user will get in-place directions over the real world as seen through the phone camera. While this constant flow of instructions is very useful, limiting its use minimises potential risks associated diverting user attention in outdoor environments~\cite{rovira2020guidance}.

%exhibiting signs of disorientation
The design of the route training component incorporates recovery features to cope with unexpected situations. Situations such as getting off track, or losing signal can be detected by checking phone sensors (GPS) and comparing the path described by the user against the route definition. Users can also explicitly report unexpected situations (e.g., road blocked, experiencing negative feelings). To these situations, the system will provide contextual and actionable assistance to either get back on track, or request help.

In terms of data collection, the training component will collect information about user location, interaction with instructions prompts and modalities, as well as unexpected situations for building performance metrics. These signals are also shared in real time with the monitoring component to enable remote assistance. For transparency, the user is informed before each practice session of the information collected, and is requested to grant permissions. Whether to allow users to deny permissions is still a contested features as we will see in the preliminary evaluation.



\fakeSection{Monitoring and assessment} 
The training process comes full circle with the \textit{monitoring and assessment} of the user progress. The main goal of this phase is to enable the remote monitoring and assistance of users during the route training, and facilitate the progress assessment and adaptation of the training for future training sessions.


{\color{red}
The monitoring 
enable real time remote assistance
and to react to calls for help

To support the assessment and adaptation the key is derivation of performance indicators.
general and broken down by sub paths 

- reliance on support (autonomy)
- ability to make correct wayfinding decisions (accuracy)
- mistakes (and unexpected situations) on track (error)
- ability to self-recover (recovery)

This is compared against the previous performances of the user.

Visualisation to simply spot parts of the route where the user is making progress and the problematic parts.



The system supports the adaptation
human in the loop.
% Metrics based on the user goal. Initially based on explicit signals (the quizes the user is getting right) and adverse events (wrong turns).

This aspect is still being developed
envision recommendation algorithms. 



}




% Do we have architecture as a separate section?

==> sections/introduction.tex <==
\section{Introduction}

The ability to move independently is a critical skill for people with cognitive impairments (CI)~\cite{wolf2021mobilitatsbildung}. It can be a catalyst for performing daily living activities, staying physically active, developing social relationships and having a higher quality of life \cite{slevin1998independent}. 
%mobility challenges?
However, people with CI face several challenges to independently and safely move around. Difficulties associated with \textit{cognitive processes}, e.g., learning the required mobility skills, spatial navigation, \textit{accessibility of navigation aids}, e.g.,  understanding maps and other traditional navigation abstractions \cite{slevin1998independent}, and \textit{social and environmental factors}, such as overprotecting parents and institutional barriers \cite{slevin1998independent}, are just some examples of such difficulties. 
% 
As a consequence, individuals with CI find themselves limited in their ability to move independently, which can lead to  sedentary behavior \cite{duggan2008impact}, have a negative impact in their psychosocial wellbeing \cite{teipel2016information} and general health [x]. Mobility difficulties also make it unsafe to move around which can lead situations such as injuries or people getting lost \cite{bantry2015dementia}.


People with CI typically have mobility resources available to them.
Help from caregivers, as well as specialised riding services, provide valuable mobility support [x]. However, this type of support puts burden on family and communities [x], and ultimately it does not address independent mobility issues.  Technology, on the other side, has the potential to support independence. While, traditional navigation technology such as Google Maps, do not meet needs and abilities of people with CI [x], research has explored specialised navigation solutions, offering metaphors and interface modalities adapted to this population [x]. 
%
For a population with limited navigation skills, training it is regarded as a proper strategy, so as not to further suppress the development of such skills~\cite{brown2011designing,oliver2008learning}. 

% family and caregivers
% some driving services for people with disabilities, which might be free depending on the community.
% Provide great service 
% Burden on communities and does not address independent mobility issues.
% Technology, navigation technology such as Google maps do not meet needs and abilities, but led to the design of several navigation technologies, which offer metaphors and interface modalities adapted to this population.
% However, training argued as the proper strategy not to further suppress navigational skills in a group with already limited skills in this regard \cite{brown2011designing,oliver2008learning}. 


% strategies to cope

% - fall back to driving services for the disabled

% - help of family or friends

% - navigation

% - training.

% why training?
% training argued as the proper strategy not to further suppress navigational skills in a group with already limited skills in this regard \cite{brown2011designing}. 

% What is mobility training?
Orientation and mobility programs aim at training individuals in concepts, required skills and techniques to integrate sensory information, spatial orientation and movement to enable safe and independent mobility~\cite{chang2020orientation}. 
Aspects commonly addressed in mobility training with people with CI include pedestrian education, use of public transportation and route learning~\cite{wolf2021mobilitatsbildung,brown2011designing,freina2015mobile,covaci2015assessing}.
This practice is commonplace with individual with vision impairments but less widespread and formalised among individuals with CI~\cite{wolf2021mobilitatsbildung}. 
%
This is further evidenced, as we will see, by the few works on mobility training support in the literature, as well as the insights derived from our extensive field work.  

% The training for 
% pedestrian education
% use of public transportation
% route learning. 

In this work we describe the \textit{design} and \textit{development} process of a mobility training system for people with CI. We focus on the specific challenges and opportunities of delivering mobility training in \textit{residential settings}, i.e.,  residential communities designed to foster and provide services for individuals with CI. 
%In this context, individuals with CI are under the care..
This is an unexplored socio-technical setting in mobility training that requires special attention to existing organisational practices, resources and limitations to ensure software solutions can be effectively adopted by individuals and inserted in the organisational environment. 
It is important to note that due to the heterogeneity of the population in the context under study, we do not take specific clinical categorisations of cognitive disabilities but rather adopt a functional perspective. As in prior work~\cite{hu2015investigating} we consider as individuals with CI those with cognitive impairments affecting mobility. 


% stakeholders with different incentives,
% knowledgeable but scarce staff,
% existing practices and protocols, 
% and heterogeneous population of individuals.
%Developing solutions for organisational rather than personal spheres shape not only system design but also the methodology applied.
%From a methodological perspective, it also raises interesting challenges to the integration of human-centered approaches and software development processes to address vulnerable populations~\cite{baez2018agile}. 

%We followed a combination of agile and human-centered approaches to go from user needs to a general technology design and prototype. Through  field visits, interviews and participatory activities, we develop a concept technology.  in two organisations in Germany


% insert new practices in organisations
% deal with limitations and resources
% heterogenous 




Through extensive user research activities with two prominent residential facilities in \textit{Anonymised}, we uncover the barriers, design challenges and requirements for mobility training in organisational settings. These informed the concept of an adaptive training system, which was developed in shorter design and development cycles. The resulting system, namely PAGAnInI, aims at enabling individuals with CI to follow a personalised route training program that can adapt to their goals, abilities and learning progress, while lowering the barriers to implementing mobility training in organisational settings. In this design and development process, we address the following research questions: 

\begin{itemize}[leftmargin=13pt,topsep=5pt]
    \item What are the main barriers, practices and design challenges to introducing mobility training in residential settings?
    
    \item How do we design a mobility training system to address individual and organisational needs and challenges?
    
    \item What methodological aspects need to be considered when engineering mobility solutions for residential settings?

    
\end{itemize}

In what follows we present the related work, design and development activities that were performed to address those questions.
% perhaps talk about the value and benefits of the insights?



%The main contributions of this work are 
% - exploration on residential settings, challenges
% - design and prototype system
%We further contribute with insights into the challenges of integrating of human-centered approaches and software development processes to address vulnerable populations




%In the organisations, mobility training has so far taken place spontaneously, irregularly and without a pedagogical concept. Many of the pedagogical staff have little space in their daily routine to carry out mobility training on a continuous basis. This is where PAGAnInI comes in. On the one hand, PAGAnInI aims to create an additional offer for people with cognitive impairments, that means to promote autonomous mobility, and on the other hand to make a contribution to technical inclusion.


% The Project "Personalized Augmented Guidance for the Autonomy of People with Intellectual Impairments" (short: PAGAnInI) addresses the intersection of participatory technology design, technology introduction and transformation research. The interdisciplinary BMBF project (duration: 2019-2023) pursues three interlinked objectives: 
% a) Firstly, a smartphone-based learning system (based on augmented reality) is being developed in participatory collaboration with people with cognitive impairments, with the help of which users should be able to move as independently as possible in public spaces. Based on an initial guided tour of a route, the system is to use machine learning to detect (in)safety in subsequent path management and adapt assistance accordingly. Ultimately, technical dependencies on the system are to be avoided and people with cognitive impairments are to be enabled to cover their routes - such as the way to work - autonomously; in the end, completely without technology. 
% b) Secondly, the organisational changes in the field are to be critically accompanied and analysed. First, the initial organisational conditions were reconstructed in a preliminary study. During the introduction of the system, it will be examined how the practices in the accompanied organisations change and which (new) patterns may emerge. 
% c) Thirdly, an essential goal is to examine the cooperation between socio-educational professionals, researchers and clients in order to analyse how participatory research with people with cognitive impairments can be designed and where obstacles lie. 

% \cite{hu2015investigating}
%  categorizations of cognitive disabilities can vary greatly
%  but as in previous research we take a functional perspective in relation too the cognitive abilities affected by the task at hand, in this case mobility.
 
%  We also provide some methodological lessons learned


%  Focus on cognitively impaired users living in residences...
%  which require a specific understanding of structures involved...

==> sections/methodology.tex <==
\section{Methodology}

\begin{figure*}[ht!]
  \centering
  \includegraphics[width=.8\linewidth]{figures/paganini-methodology.pdf}
  \caption{Methodological approach. A \textit{pre-requirements} phase to get insights on the complex problem space, a main \textit{design and development} process, featuring design sprints one step ahead of development, and the \textit{deployment} of the technology in context. The concentric circles illustrate the main conceptual iterations in terms of focus of the process:  (1) concept development, (2) experience prototyping and (3) development and refinement of software artefacts.}
  \Description{Methodological approach and associated activities}
  \label{fig:methodology}
\end{figure*}

 We followed a \textit{human-centered} agile development approach, adopting strategies from the literature to integrate product discovery, design and development to engineering solutions for vulnerable populations~\cite{baez2018agile,brhel2015exploring,carroll2016aligning}. In terms of the process, we integrated user research activities as a pre-requirement phase (e.g., as seen in \cite{carroll2016aligning}) so as to get an understanding of the users and the complexity of the problem space before diving into the design and development. After this preliminary phase, we run parallel design and development interwoven tracks, allowing design cycles at least one sprint ahead to inform subsequent developments~\cite{brhel2015exploring}. We conceptually went through three main phases in the design and development, from (1) \textit{concept development}, aiming at shaping the overall focus and concept of mobility training support to (2) \textit{prototyping the experience} of using the technology, involving users in the forseen training process  to (3) \textit{producing design and software artifacts} of different level of maturity.
We summarise the methodology in Figure~\ref{fig:methodology}.

\fakeSection{User activities.}
The type of activities and the of level involvement was tuned to allow for a wide rage of feedback from people with cognitive impairments, which is emerging as an important aspect of inclusive design practices \cite{spencer2020including}. Among the methods we employed we can mention: 
%direct interviews with users, technology probes, experience prototyping with incomplete prototypes, and proxy activities with other stakeholders (e.g., caregivers). In the following we summarise the main activities: 

\begin{itemize}[leftmargin=13pt,topsep=5pt]
\item \textit{Preliminary visits}. We approached interest groups and organisations with the purpose of getting a better understanding of the entire context and establishing partnerships with organisations interested in participating in the project. We partnered with two main organisations in \textit{Anonymous}, which gave us access to residential facilities and sheltered workshops for people with disabilities. We held meetings with different stakeholders to help us establish a working approach and strategy to the collaboration.

\item \textit{Interviews}. We carried out semi-structured interviews with individuals with CI as well as professionals (e.g., rehabilitation managers, caregivers), in order to get insights into the barriers, needs and opportunities for mobility training in the target scenario. What emerged from this and the previous activity, are insights and requirements that shaped the concept design of a route training application.

\item \textit{Concept validation.} The technology concept of the route training application was then validated with users and professionals, who assessed main components of the solution in scenario-based interviews driven by storyboards.

\item \textit{Experience prototyping.} We prototyped the main route training process and activities by relying on technology probes~\cite{hutchinson2003technology} and partial working prototypes of the system. This emerged as a necessary and effective way of eliciting (more) specific feedback from our target users.


\item \textit{Formative design studies.} We performed formative design feedback sessions with prototypes of varying level of detail, from paper to high-fidelity prototypes, focusing on:  understanding of UI and navigation \textit{metaphors} (e.g., symbols, icons), \textit{accessibility} features (e.g., colors, fonts), and \textit{organisation} and usability of specific system components (e.g., training component).



%\item \textit{Pilot trials}

\end{itemize}



%[x] to go from user needs to a general technology concept and design. From a software engineering perspective, this process was akin to having a preliminary user research phase to understand the complexity of the users and scenarios, followed up by design and development sprints to bring down the concept into concrete prototypes. 

\fakeSection{Design and software artefacts.}
The design and development process led to the generation of artefacts of varying level of maturity, from 
\textit{personas}, which captured our specific target user, \textit{storyboards}, which help us illustrate the concept of route training putting personas in specific target scenarios, \textit{mockups} from paper-based to high-fidelity ones to get more input of the user experience design directions, and \textit{working prototypes} to support pilots with actual system components.

\fakeSection{Team composition.}
The project is carried out by a interdisciplinary team with expertise in the different relevant aspects, including: three \textit{social scientists} with training in human-subjects research and mobility training, who led and carried out the field activities; two \textit{designers} with expertise in design methods and prototyping tools, who supported the design activities; two software \textit{engineers} with expertise in agile methods and the development frameworks used in project. To ensure smooth coordination of team members of diverse background, the team included one researcher with multidisciplinary background with expertise in engineering solutions for vulnerable groups that acted as a \textit{cross-functional} team member~\cite{baez2018agile}. We also involved software engineers as observers in certain user activities as a way to empathise with the users.
%
The project also relied on external consultations with \textit{privacy} and \textit{legal} experts to account for missing expertise in the core team.

\fakeSection{Ethics and advisory board.}
One specialised expert panel have been appointed to oversee the research and strengthen the quality of the results. 

\textit{The ethics committee}. The ethics committee consists of 5 persons representing all status groups in the project: 2 researchers with expertise in accompanying people with disabilities; 2 people with disabilities from institutional living and working contexts and 1 inclusion planner from the city administration.
Interim results are presented to the ethics committee at regular meetings throughout the project and ethical implications are discussed together during the research process (e.g. on participation) and afterwards (e.g. on the use of digital assistive technologies). 
The research team and the ethics committee have agreed on an evaluation concept for the gradual testing and subsequent adaptation of the system in order to be able to assess the effectiveness, usability and suitability for everyday use (from a sociological as well as a technical point of view) in the pilot phase. 

% In our Project, we followed a human-centered design approach. Based on this approach, different steps have been taken so far.The preliminary user research phase includes interviews with 15 people and several observations of the everyday life and the mobility. A special feature of the interviews with the users was that photos of paths or buildings were used early on in order to work out points of orientation. The interviews were then analysed using social science methods. Afterwards, the categories were cast into personas and user stories were created. On the basis of the personas and the user stories, first analogue mock-ups for the people with CI could be created.  In iterative loops, we worked together with the users to further develop the design until a first prototype could be developed. This prototype was tested again in practice, together with the people, evaluated and further developed. 

% The project team was composed of 
% social scientist
% designers
% engineers 

% external consultations with privacy and legal experts(?)


% We followed a human-centered design approach [x] to go from user needs to a general technology concept and design. From a software engineering perspective, this process was akin to having a preliminary user research phase to understand the complexity of the users and scenarios, followed up by design and development sprints to bring down the concept into concrete prototypes. 


% from the user research we have two main activities

% \begin{itemize}
%     \item Preliminary visits to relevant stakeholders and organisations
%     \item interviews with CI individuals and social workers
%     \item design and development activities
%     \item formative feedback
% \end{itemize}

% team composition

% ethics

\smallskip
\noindent In this paper we early stages of the design and engineering, from the understanding of user needs and elicitation of requirements, to the initial validation of the concepts and development of early working prototypes.

==> sections/related.tex <==
\section{Related Work}

\fakeSection{Mobility training for people with CI}
% how people with intellectual disabilities is different from other populations?
The design and development of technology-supported mobility training for cognitively impaired individuals has been investigated in three prominent research projects.

RouteMate~\cite{brown2011designing} is a route learning system for people with intellectual disabilities developed in the context of the RECALL project. The approach is based on scaffolding the learning of new routes, i.e., going through different levels of support until reaching independent mobility. A mobile app for the CI users thus offers training of map-based concepts in three different modes. The \textit{planning} mode, where a route (start, destination) is defined with the help of a trainer, and augmented with POIs (enriched with text, pictures and symbols), a schedule for routine walks, and emergency contacts. The \textit{practice} mode allows the user to rehearse the prepared route, and offers location-based reminders when getting close to POIs, alarms  (visual and haptic) when deviating from the defined routes. In the \textit{use} mode the user is encouraged to use their own skills through the gamification of the route navigation. The screen turns off while navigating between POI, and when reaching one, users are challenged to select the picture that corresponds to the POI. A pilot study with 8 intellectually disabled participants \cite{brown2013engaging} showed a reduction of errors from practice to use mode after one session but this gain was not statistically significant.
The RouteMate system was then further developed in the direction of game-based learning \cite{brown2013engaging}. The use mode was replaced with a \textit{challenge} mode, which incorporated digital scavenger hunts (e.g., a ninja-game route) that aimed at reinforcing map concepts and route learning. Qualitative results from pilots suggest that participants were better at retaining information in a game setting.

% focus on maps, containing complex representations and symbols that require abstraction (not our target users)
% two modes, no intermediate learning steps
% the process does not account for how paths are personalised
% limited modalities for the instructions
% limited technology-mediated support offered by trainers, who can only intervened in response to calls.

% Challenge mode
% game-based
% ninja-game route 
% narrative game structure
% scavenger hunt where users had to collect diamonds that were unlocked when predefined points in the route where reached, and were given to the user who could recall that stop at the end of the session.
% making it fun, encourage concentration and contribute to spatial map formation.
% Qualitative results suggested that participants were better at retaining information in a game setting.


% type of navigation?
% type of learning
% plan mode
% a route is defined with the help of a caregiver, parent or trainer.
% - start and destination 
% - points of interest along the way to break the journey in smaller routes connected by key landmarks to make learning effective
% - emergency contact
% - time sensitive walks (schedule)
% - text, photo and symbols
% user navigates a prepared route
% the system

% practice 
% - location based reminder when getting close to a point of interest (pictures)
% - alarms when deviating from route
% - visual and haptic alarms

% Use mode
% the user is encouraged to use their own skills through the gamification of the route navigation. 
% - user quizzed on the next point of interest, where the user is challenged to select picture associated to the POI from the pictures defined during the planning. - screen turns off while navigating between POI
% - when arriving to the destination, provides information about the time taken and invites the user to reflect on the journey.


% \cite{brown2013engaging}


% focus on map learning
% a study with 8 intellectually disabled participants show a reduction of errors from practice to use mode after one session but these were not statistically significant

% Challenge mode
% game-based
% ninja-game route 
% narrative game structure
% scavenger hunt where users had to collect diamonds that were unlocked when predefined points in the route where reached, and were given to the user who could recall that stop at the end of the session.
% making it fun, encourage concentration and contribute to spatial map formation.
% Qualitative results suggested that participants were better at retaining information in a game setting.

% focus on maps, containing complex representations and symbols that require abstraction (not our target users)
% two modes, no intermediate learning steps
% the process does not account for how paths are personalised
% limited modalities for the instructions

The SmartAngel \cite{freina2015mobile} project aims at enabling subjects with intellectual impairments, and particularly individuals with Down Syndrome, to move around independently in a urban context. The project developed a set of applications providing support in two steps: a \textit{pre-training} phase where navigation-related skills are trained in a simulated environment and a second phase, where  \textit{on-the-street} support is provided for actual route navigation. The pre-training phase apps aim at addressing the longer training time required due to learning challenges by reducing the on-the-street training. One of such apps, namely FriendlyRoad \cite{freina2014learning}, provides a virtual environment where the user can safely  train mobility skills associated to street dangers before moving onto actual streets. Unlike the traditional approach based on a theoretical training and multimedia material, the adopted 'experiential learning' approach  offers the virtual immersive experience to address transfer learning issues and allow for a systematic training of different scenarios. 
%Other apps developed cover aspects such as spatial orientation \cite{bottino2014smart}.
%
The on-the-street support \cite{freina2015social} provided is essentially a monitoring system. It targets individuals with CI that already have the ability to move independently in known areas, monitoring their walks in real time and acting as a safeguard so that tutors can support and intervene when needed.

% a monitoring system for tutors
% as the user beings more independent the monitoring system acts as a safeguard to support and intervene when needed.
% real time information
% targeted at individuals that already have the ability to move independently in known areas.
% account for unplanned situations

%The system does not support training in the sense of route learning. It target general skills and individuals who can already move around in known places, providing for these monitoring..


% FriendlyRoad \cite{freina2014learning}, 
% individuals with Down Syndrome
% difficulty in transferring learned skills in a different situation,  environment or future experience
% learning requires longer time

% focused on street dangers

% how:
% providing a virtual environment where the user can safely traing before moving into the real streets.

% goal: reduce the on the street time training and risk of accidents

% the traditional approach is based on a theoretical training level, through multimedia material. focused on safety
% problem is this training is not on the road, leading to transfer problmes
% and even when the taining moves to the road, not all scnerios can naturally occur.

% guided experiencial learning rooted on repetition

% the concept: is a serious game based on a virtual immersive environment .

% later adapted to older adults with dementia

% spatial orientation \cite{bottino2014smart}

% All the games are developed to be played by the target users in the presence of a tutor

% \cite{freina2015social}
% On the road supports

% a monitoring system for tutors
% as the user beings more independent the monitoring system acts as a safeguard to support and intervene when needed.
% real time information
% targeted at individuals that already have the ability to move independently in known areas.
% account for unplanned situations

% The system does not support training in the sense of route learning. It target general skills and individuals who can already move around in known places, providing for these monitoring..


The POSEIDON (PersOnalized Smart Environments to increase Inclusion of people with DOwn’s syNdrome) project \cite{covaci2015assessing} also explored mobility training for CI individuals.  The project developed solutions for training and navigation support for individuals with Down Syndrome. A \textit{stationary system} \cite{covaci2015assessing} provided a VR environment, where scenarios could be systematically manipulated for individualised training. In this system, a virtual trip is customised and enhanced by a caregiver, with landmarks, points of interest and dangerous points. The trainees would then learn and rehearse the route in the virtual environment. A \textit{mobile app} \cite{kramer2015developing} would then support the navigation of the actual trip on the streets. The mobile app displays the route definition of the stationary system, relying on map representations and picture aids. Caregivers can monitor trainees but do not interfere with the navigation. Results from pilots indicated problems reading the map, translating instructions into actual movements, and standard directional assistance from off-the-shelf systems not covering all their needs.
% offers pre-training and would be complementary to ours
% our approach is based on experiential learning on the streets
% path definition are based on personalised and negotiated
% we provide actual support during training and not just navigation

% \cite{kramer2015developing}
% - light version, mobile app to support the actual navigation (just navigation with no specific training objectives in place)
% caregivers can monitor but not interfere?
% displaying route definition of the stationary system
% uses a map and pictures
% results from pilots show that problems reading the map, translating instructions into actual movements, and standard directional assistant from off-the-shelf system not covering all their needs, 

%The POSEIDON (PersOnalized Smart Environments to increase Inclusion of people with DOwn’s syNdrome) project \cite{covaci2015assessing}
% training and support of navigation for individuals with Down Syndrom
% relies on VR as a way to create environments where scenarios can be systematically manipulated for individualised training

% two components
% - a full system, stationary \cite{covaci2015assessing}
% VR
% learn and rehearse aspects of a route
% the virtual trip is customised and enhanced by the caregiver. Additional annotations on the route include: landmarks, dangerous points, and points of interest

% \cite{kramer2015developing}
% - light version, mobile app to support the actual navigation (just navigation with no specific training objectives in place)
% caregivers can monitor but not interfere?
% displaying route definition of the stationary system
% uses a map and pictures
% results from pilots show that problems reading the map, translating instructions into actual movements, and standard directional assistant from off-the-shelf system not covering all their needs, 



\fakeSection{Wayfinding and navigation technologies} 
Another relevant category of technology support is wayfinding and navigation. Although these systems do not support training, they do explore mechanisms to relay navigational instructions to CI individuals, which can inform the on-the-street support. 
% Important aspect to analyse in this regard are the type of route mobility supported
% how the routes and instructions were generated
% what type of adaptations are supported
% and the modality of instructions

% modality
% type of mobility support
% calculated vs designed
% adaptation

Three prominent types of mobility approaches have been implemented and evaluated with CI individuals. 
\textit{Directional awareness}, where the idea is to  aid basic orientation tasks through a digital compass. This approach was explored in the Home Compass app~\cite{rassmus2014finding}, which aimed at supporting older adults with memory declines to freely move in their neighborhoods while keeping a reference point to home. \textit{Landmark-based navigation} where the idea is to rely on landmarks along a route as primary means of providing direction and supporting decisions. This navigation approach has been implemented in several systems, such as the NavMem system~\cite{poppinga2014navmem} supporting wayfinding for individual with memory declines, by breaking a navigation task into simpler tasks by leveraging landmarks with visual cues (pictures).  %AssisT-OUT~\cite{gomez2015adapted} follows a similar approach supporting wayfinding for pedestrian with cognitive disabilities by leveraging street-level photos from Google Street View at decision points. 
\textit{Turn-based navigation}, that aim at providing specific turn-by-turn navigation instructions to users. This approach is implemented in general-purpose navigation systems, and has been explored in some navigation for CI individuals, such as the handheld AR-based system by for Ramos et al. \cite{ramos2013geo} aiming at providing turn-by-turn direction overlaid on the mobile phone camera.
%
Previous studies [x] involving these approaches indicate that landmark-based navigation to be the preferred, less cognitively demanding and most effective one for CI individuals. 



% \textbf{type of route mobility supported}

% orientation / compass
% %NavMem Explorer: An Orientation Aid for People with Mild Cognitive Impairments
% \cite{poppinga2014navmem}
% %[2014] Finding the Way Home – Supporting Wayfinding for Older Users with Memory Problems
% \cite{rassmus2014finding}

% turn-based
% %[2013] Geo-localization System for People with Cognitive Disabilities
% \cite{ramos2013geo}
% generated
% AR for the routing
% monitoring for the caregiver
% a travel pathdesigner but only to specify destinations
% (instructions are calculated)


% path is planned
% wayfinding with remote monitoring (and planning)
% %[2015] An Adapted Wayfinding System for Pedestrians with Cognitive Disabilities
% \cite{gomez2015adapted}
% landmark based

{\color{red}
The personalisation of the the route navigation is implemented at different degrees. 
- No personalisation:  landmark and instructions extracted from out-the-shelf directional systems with no specific personalisations \cite{ramos2013geo}
- Route designed by caregivers \cite{gomez2015adapted}
- No specific support for involving users in the design of routes
--- Insights into what is best? Quality of landmarks have an impact.

% \textbf{Generation of instructions}
% path is planned
% wayfinding with remote monitoring (and planning)
% %[2015] An Adapted Wayfinding System for Pedestrians with Cognitive Disabilities
% \cite{gomez2015adapted}
% landmark based


\textbf{Modality and presentation of instructions}

AR
%An Assistive Navigation System Based on Augmented Reality and Context Awareness for People With Mild Cognitive Impairments
\cite{hervas2013assistive}

% [2012] A Friendly Navigation-System Based on Points of Interest, Augmented Reality and Context-Awareness
\cite{ma2012friendly}




\textbf{adaptation}

adaptation
%[2017] GAWA – Manager for accessibility Wayfinding apps
\cite{rodriguez2017gawa}


to support the promotion of physical activity
%[2021] HikePal_ A mobile exergame to motivate people with intellectual disabilities to do outdoor physical activities
\cite{torrado2022hikepal}
%[2020] Developing Software for Motivating Individuals with Intellectual Disabilities to do Outdoor Physical Activity
\cite{torrado2020developing}

}

==> sections/requirements-table.tex <==

\begin{table*}[htp]
%\vspace{-0.2 cm}
\small
\caption{Requirements}
\label{tab:themes}
\begin{tabular} {p{0.65\textwidth} p{0.30\textwidth} }
\toprule
\textbf{Requirement} & \textbf{Solutions}\\
\midrule

     \textbf{Training supervision \& monitoring}
     
    [R1] \textit{Support route learning not just navigation}. Mobility support should assist individuals with CIs in route learning, not just provide directional instructions. %left, right, left… (not google maps)
    
    [R2] \textit{Keep the expert in the loop}. Professionals have accumulated knowledge and expertise, so it is crucial to support them (and their practices) in the training rather than replacing them. %It is important that the system does not replace personal attention. 

    %\item [R] time management - specific feature (under goals)
    [R8] \textit{Provide transparency, protection and control over user privacy and data}, especially for the monitoring. It is important that users are made aware of the implications of data sharing, its purpose, and provide control mechanisms to turn it off.     

    & Route training 

    \textbf{Personalisation}
    
    [R3] \textit{Allow for the adaptation of the training to the individual goals and progress}. It is fundamental to account for the different situation of the individuals, their goals in terms of route training, and to incrementally adapt the training to their learning progress.

    [R7] \textit{Account for people's different abilities to learn and interpret instructions}. Given the diversity of the target population in terms of abilities, the system should be adaptable to the modalities (e.g., visual, audio) and representations (e.g., text, pictures, signs) that are more effective in guiding and training users.   

    [R9] \textit{Make the system accessible and usable}. Differences in interaction abilities should be taken into account to design an accessible system that can be effectively used by a wider set of individuals.     


    \textbf{Practice support}
    
    [R4] \textit{Make the mobility support safe to use}. The solution should consider safety of use by design, minimising the attention required by the system and avoiding distractions in traffic. 
    
    [R5] \textit{Address negative feelings} associated with the training. Feelings of uncertainty and fear of getting lost, should be reduced by incorporating design elements that address them at the source. 
    
    [R6] \textit{Incorporate safety nets in case of unexpected situations}. The system should account for unexpected situations that can arise due to human and technology errors, and changes in the environment, and provide mechanisms to recover from them. 
    
    
    


    


\bottomrule
\end{tabular}
\end{table*}  

